Detecting and Measuring Security Implications of Entangled Domain Verification in CDN

Content Delivery Networks (CDNs) offer a protection layer for enhancing the security of websites. However, a significant security flaw named Absence of Domain Verification (DVA) has become emerging recently. Although this threat is recognized, the current practices and security flaws of domain verification strategies in CDNs have not been thoroughly investigated. In this paper, we present DVAHunter, an automated system for detecting DVA vulnerabilities that can lead to domain abuse in CDNs. Our evaluation of 45 major CDN providers reveals the prevalence of DVA: most (39/45) providers do not perform any verification, and even those that do remain exploitable. Additionally, we used DVAHunter to conduct a large-scale measurement of 89M subdomains from Tranco's Top 1M sites hosted on the 45 CDNs under evaluation. Our focus was on two primary DVA exploitation scenarios: covert communication and domain hijacking. We identified over 332K subdomains vulnerable to domain abuse. This tool provides deeper insights into DVA exploitation and allows us to propose viable mitigation practices for CDN providers. To date, we have received vulnerability confirmations from 12 providers; 6 (e.g., Edgio, Kuocai) have implemented fixes, and 1 (ChinaNetCenter) are actively working on solutions based on our recommendations.

==> Sections/3.design_and_implementation_bak.tex <==
\section{Design and Implementation}

\subsection{Motivation}
DVA vulnerability is prevalent in CDNs, posing significant threats to the integrity and security of the Internet. 
Despite efforts by previous researchers ~\cite{domain_fronting,domain_borrowing_bh,takeover_xyz} to mitigate the DVA vulnerability, security incidents continue to occur. APT29 (also known as Cozy Bear) reportedly exploits domain fronting to disguise its C2 (Command \& Control) of malware or botnet infrastructure, thereby complicating detection and attribution \cite{tor_meek}. Another study~\cite{CCTV}  reveals that attackers utilize domain borrowing to bypass network detection, borrowing the reputation of a legitimate domain to distribute RT malware. What is worse, researchers~\cite{Microsoft_takover} have discovered hundreds of dangling Microsoft subdomains, allowing attackers to take them over through Microsoft Azure.

With a comprehensive analysis of previous works, we identify two research gaps in detecting DVA vulnerability. Firstly, there is no universal method to identify vulnerable CDN providers. The CDN providers offered domain connection policies are highly diverse~\cite{hosting_service}, and there are no uniform features to identify vulnerable CDN providers. Secondly, given the large number of CDN providers and the millions of domains, the accurate detection of vulnerable CDN providers and the timely exposure of vulnerable domains poses a significant challenge. In a word, there is still no automatic detection system to identify DVA vulnerability.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]
    {images/./figures/crop_system_v16.pdf}
    \caption{\toolname workflow.}
    \label{fig: workflow}
\end{figure*}

\subsection{System Overview}
To fill the research gap in detecting DVA vulnerability, this study designs and implements \toolname to evaluate its severity automatically and periodically at the Internet scale.
As shown in Figure~\ref{fig: workflow}, \toolname consists of three key components: (1) Subdomain Crawler, (2) CDN Checker, and (3) Domain Verification Checker. First, the Subdomain Crawler enumerates subdomains of the targeted domains. 
\lzy{Second, the CDN Checker crawls DNS records, collects ingress node IPs, and discovers domains hosted by CDNs for further domain verification checking. Third, the Domain Verification Checker automatically detects DVA vulnerability based on the information collected by the first two components. }
We will elaborate on the role of each system component.

\subsection{Subdomain Crawler}
We use a custom prefix dictionary to generate a list of Fully Qualified Domain Names (FQDNs) under the Second-Level Domain (SLD), offering greater flexibility in our subdomain discovery process~\cite{subdomain_crawler}. Each prefix is joined with the target SLD to create an FQDN. Then, we validate the existence of these FQDNs using DNS queries. During the verification process, we send query requests to DNS servers to check whether there are corresponding resource records for the FQDNs we created. If the DNS response contains valid records, it indicates that the FQDN exists under the target SLD. To filter out wildcard DNS records, we also include a random prefix in our queries to identify and exclude. Through this approach, we can detect valid FQDNs under the target SLDs and expand the scope of our search.

\subsection{CDN Checker}

We have developed the CDN Checker to provide comprehensive domain data for Domain Verification Checker. The CDN Checker comprises three components that collaborate to conduct thorough domain scanning. These components are (1) Crawling DNS records, (2) Discovering domains hosted by CDNs, and (3) Collecting ingress node IPs.



\noindent \textbf{Crawling DNS records.}
We crawl CNAME, NS, and A records. To accelerate the DNS records crawling time for Tranco Top 1M domains, we concurrently launch five instances of our DNS crawler that would start from different indexes in Tranco Top 1M domains. It took approximately one day to finish the scan. 

\noindent \textbf{Discovering domains hosted by CDNs.}
When domain owners want to deploy their domain on a CDN, the CDN assigns a subdomain belonging to the CDN itself. The domain owner must create a CNAME record pointing their domain to the CDN-assigned subdomain to redirect traffic to the CDN. We can identify domains hosted by a CDN by following the steps.
\lzy{Firstly, for a given CDN (e.g., Fastly), we gather CDN-assigned subdomains from a publicly available paper~\cite{cdn_dark_side} and further supplement it using the Public Suffix List~\cite{public_suffix_list}. Secondly, we compare the previously collected DNS records with the CDN-assigned subdomains (see Table~\ref{table: cdn_assigined_subdomain}) to identify the domains hosted on the CDN. Thirdly, we send HTTP requests to the identified domains hosted by the CDN. We then compare their responses with non-CDN-deployed fingerprints (see Table~\ref{table: non-CDN-deployed fingerprints}) to recheck the domains hosted by the CDN. This rigorous process ensures the accuracy of our results, clearly distinguishing between CDN-deployed and non-CDN-deployed domains that reduce false positives. Finally, we categorize these domains based on the CDN provider for further in-depth analysis.}


\noindent \textbf{Collecting ingress node IPs.} 
We need CDN ingress node IP addresses to detect domain borrowing. 
The accuracy of them determines the success rate of detecting domain borrowing. Unfortunately, to the best of our knowledge, CDN ingress node IP addresses are not fully publicized on the Internet. Therefore, we need to collect the ingress node IP addresses of CDN by ourselves. Internet-wide scan is a traditional method of collecting the ingress node IPs. Send an HTTP request to the Internet-wide IPv4 space that sets the well-known CDN customers' domain as the Host header. If the response is the correct web page, which indicates the IP is the ingress node IP. However, this method cannot filter out open proxies. We have found that ingress node IPs can be gathered by querying DNS resolvers for CDN customer domains~\cite{measuring_cdn,imc_2013,sigcomm_2015}. 
Firstly, we compare the previously collected DNS records of the domain with the CDN-assigned subdomain to gather the domain hosted by CDNs. Secondly, we gather the CDN-hosted domain' A record as the CDN ingress node IPs. Thirdly,  we need to filter these IPs to ensure their validity. We conduct a liveness check by sending HTTP requests and waiting for their responses. If a node fails to respond, responds slowly, or responds without the specific HTTP header (e.g., ``Server: cloudflare''), we consider it unavailable and remove it from the list. Fourthly, due to the large size of the CDN, the number of ingress node IPs can be very significant. We classify the ingress node IPs using GeoIP data. Based on this data, we categorize the ingress node IPs according to their city locations. Finally, we randomly select one IP from each city and combine these IPs into a list. This list represents the globally distributed CDN ingress node IPs. 

\begin{table*}[ht]
    \caption{CDN-assigned subdomain.}
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{@{}ll|ll@{}}  
    \toprule[1.5pt]
    \textbf{CDN}            & \textbf{Assigned subdomain}                                                                     & \textbf{CDN}            & \textbf{Assigned subdomain}                                     \\ 
    \midrule

    \textbf{AligeCDN}          & agilewingcdn.com                                              & \textbf{Goooood}        & .prod.defense-dns.net                             \\
\textbf{Akamai}         & .akamai.net, .akamaiedge.net , .edgesuite.net                               & \textbf{HuaweiCloud}         & .cdnhwc1.com, .cdnhwcxcy07.com.                   \\
 \textbf{Alibaba}        & .cdngslb.com, .alicdn.com, .alikunlun.com, .kunlunsl.com                                        & \textbf{JDCloud}        & .cloud-scdn.com, .jcloud-cdn.com,                 \\
\textbf{ArvanCloud}     & .arvancdn.com, .arvancdn.ir                                                            & \textbf{KeyCDN}         & .kxcdn.com, .kvcdn.com                            \\
\textbf{Azion}          & .map.azionedge.net, .azioncdn.net                                                      & \textbf{KingsoftCloud}       & .ksyuncdn.com, .ks-cdn.com                        \\
\textbf{Azure}          & .azureedge.net, .azurefd.net                                                           & \textbf{KuoCai}         & .kuocaidns.com.                                   \\
\textbf{Baidu}          & .bdydns.com, .jomodns.com, .yunjiasu-cdn.net                                           & \textbf{LeaseWeb}       & .lswcdn.net                                       \\
\textbf{BelugaCDN}      & .belugacdn.com                                                                         & \textbf{Layun}          & .yuncdn.layuncdn.com                              \\
\textbf{Bunny}          & .b-cdn.net, .b-cdn.com, .bunny.net, .bunny.net.                                        & \textbf{LightCDN}       & .r.cdn36.com                                      \\
\textbf{Cachefly}       & .cachefly.net                                                                          & \textbf{Limelight}      & .llnwd.net, .lldns.net                            \\
\textbf{CDN77}          & .rsc.cdn77.org, .cdn77.net, .cdn77-ssl.net                                             & \textbf{Lumen}          & .footprint.net, .fpbns.net                        \\
\textbf{CDNetworks}     & .cdngc.net, .gccdn.net, .qtlgslb.com, .cdnetworks.net                                  & \textbf{Medianova}      & .mncdn.com, .mncdn.org                            \\
\textbf{CDNsun}         & .cdnsun.net                                                                            & \textbf{Netlify}        & .netlify.com, .netlifyglobalcdn.com, .netlify.app. \\
\textbf{CDNvideo}       & .cdnvideo.ru                                                                           & \textbf{Qiniu}          & .qiniudns.com                                     \\
\textbf{ChinaNetCenter} & .qtlcdn.com                                                                            & \textbf{StackPath}      & .hwcdn.net, .stackpathcdn.com, .stackpathdns.com  \\
\textbf{Cloudflare}     & .cdn.cloudflare.net                                                                    & \textbf{Tencent}        & .cdn.dnsv1.com, .tdnsv6.com.                      \\
\textbf{CloudFront}     & .cloudfront.net                                                                        & \textbf{UCloud}         & .ucloud.com.cn                                    \\
\textbf{DogeCloud}      & .s2-web.dogedns.com                                                                    & \textbf{Udomain}        & .xcdn.global                                      \\
\textbf{EdgeNext}       & .bsclink.cn                                                                            & \textbf{UPYun}          & .aicdn.com                                        \\
\textbf{Edgio}          & .glb.edgio.net, .systemcdn.net, .edgecastcdn.net.                                      & \textbf{Yunaq}          & .cdn.jiashule.com                                 \\
\textbf{Fastly}         & .fastly.net, .fastlylb.net                                                             & \textbf{Yundun}         & .cname.hcnamedns.com                              \\
\textbf{G-core}         & .d.gcdn.co                                                                             & \textbf{Sudun}          & .sudun1.suduncdn.com                               \\
    \bottomrule[1.5pt]
    \end{tabular}
    \begin{tablenotes}
    \item[1] KuaikuaiCloud is a Multi-CDN that uses the infrastructure of Tencent or Baidu. So it doesn't have its own subdomain
    \end{tablenotes}
    \end{threeparttable}    
    \label{table: cdn_assigined_subdomain}
\end{table*}




\subsection{Domain Fronting Tester}
Figure~\ref{fig: workflow} shows the workflow of Domain Fronting Tester, which can be divided into three steps: (1) We utilize the previously collected domains hosted by CDNs to discover valid URLs from these domains. (2) We select domains from the same CDN provider and pair them with valid URLs to generate testing tuples. (3) We use these testing tuples to conduct domain fronting testing and verify whether the CDN provider is vulnerable to domain fronting.


\noindent \textbf{Discovering valid URLs served by CDNs.}
After identifying domains hosted by CDN, we crawl the URLs that are actual web objects on these domains. However, a challenge arises when making a direct ``GET /'' HTTPS request to ``https://www.example.com'' without specifying the complete resource path, as it may fail due to the web server not allowing access to the root directory. Therefore, we have developed a custom Chromium-based web crawler using Selenium~\cite{Selenium}. Our crawler accesses a domain and captures all network requests and corresponding responses. Domain fronting testing requires the content of a URL to remain stable across multiple requests, so we only retain URLs for static web resources such as images, .js, and .css files on www.example.com.

\noindent \textbf{Generating testing tuples.}
For testing domain fronting on a CDN, the process involves selecting a front domain (called \textit{Fd}), a target domain (called \textit{Td}) also hosted by the same CDN provider, and a URL from the target domain (called \textit{Ut}). The steps are: (1) establish a TLS connection using the \textit{Fd} as the Server Name Indication (SNI), (2) send an HTTPS request for the \textit{Ut} with the Host header set to the \textit{Td}. If the web object is successfully fetched without errors and the SNI points to the \textit{Fd}, the CDN is vulnerable to domain fronting. However, in practice, the above process is not sufficient. We also need to ensure that the object returned from an HTTPS request is identical to the web object provided by the CDN without SNI alteration. Furthermore, we also need to ensure consistent results across different domain pairs (\textit{Fd}, \textit{Td}) within the CDN to determine if the entire infrastructure is vulnerable to domainfronting. Therefore, we select up to 10 tuples (\textit{Fd}, \textit{Td}, \textit{Ut}) from the CDN. For each tuple, the \textit{Fd} serves as the SNI, the \textit{Td} hosts the \textit{Ut}, and both domains are under the same CDN provider. 

\noindent \textbf{Recognizing vulnerable CDNs.}
We processes each selected tuple (\textit{Fd}, \textit{Td}, \textit{Ut}) as follows:

\begin{itemize}

\item[$\bullet$] \textit{Step 1:} Request target URL with target domain as SNI and Host header.
We craft an HTTPS request for the URL \textit{Ut}, setting both the Host header and SNI as \textit{Td}. We store the response content as \textit{Rt}.

\item[$\bullet$] \textit{Step 2:} Request target URL with front domain as SNI and target domain as Host header. We craft an HTTPS request for \textit{Ut} but set the SNI as \textit{Fd} while setting the Host header as \textit{Td}. We store the response content as \textit{Rv}.

\item[$\bullet$] \textit{Step 3:} Request target URL with front domain as SNI and Host header. We craft an HTTPS request for \textit{Ut}, setting both the Host header and SNI as \textit{Fd}. This step verifies that \textit{Ut} is not available under \textit{Fd}, ensuring the test’s validity. We record the response content as \textit{Rf}.

\end{itemize}

By analyzing the responses in the following steps, we determined that the domain fronting tests were successful:

\begin{itemize}
\item[$\bullet$] \textit{Rt} is a valid HTTP response without errors.
\item[$\bullet$] \lzy{\textit{Rv} should match \textit{Rt}, indicating consistent behavior of the target URL when the SNI setting is the front domain, but the Host header set is the target domain.}
\item[$\bullet$] \textit{Rf} should be either empty (indicating response 404 Not Found) or should be different from \textit{Rt}, confirming that the front domain does not serve the content of the target URL when both the SNI and the Host header set as the front domain.

\end{itemize}

To compare the content of \textit{Rt}, \textit{Rv}, and \textit{Rf}, we compute and compare their SHA1 hashes~\cite{eastlake2001us}. We repeat these tests up to ten times for each CDN, with each test based on a randomly chosen tuple. After these processes, we are able to recognize all the vulnerable CDN providers.

\subsection{Domain Borrowing Finder}
Figure~\ref{fig: workflow} shows the workflow of Domain Borrowing Finder, which can be divided into three steps: (1) We identify vulnerable CDNs and collect responses of the domain non-CDN-deployed as non-CDN-deployed fingerprints. (2) We use the previously collected domains not hosted by CDN as the Host headers to generate legal HTTP requests. (3) We send generated HTTP requests to CDN ingress nodes and compare the HTTP response with non-CDN-deployed fingerprints to identify the borrowing domains.

\noindent \textbf{Identifying vulnerable CDNs.}
To identify CDN providers vulnerable to domain borrowing, we need to collect responses of the non-CDN-deployed domain. Although previous work~\cite{domain_borrowing_bh} has manually identified that five CDN providers are vulnerable to domain borrowing, there have been no systematically explored CDN providers and collected non-CDN-deployed fingerprints. Therefore, we adopt the following automated approach:

\begin{itemize}
\item[$\bullet$] \textit{Step 1:} 
\lzy{Domain verification means the person who is the domain owner and can manage the domain's authoritative server.}
Customers can claim domain ownership on a CDN provider in two ways. (1) DNS-based verification: CDN providers generate a challenge token and ask customers to configure it in a DNS record (e.g., CNAME or TXT). (2) Web-based verification: CDN providers ask customers to upload a file containing a challenge token to a specific directory on the website. Many Internet services now need domain verification but no standard practices. We inspect their domain verification mechanism as follows. Firstly, we review CDN providers’ operational documentation and search for service setup tutorial videos to find the officially claimed domain verification mechanism. \lzy{Secondly, we will register one test account for each CDN provider, create a service, and configure our server as origin.
We inspect whether the test account can set the custom domain as a high-reputation domain that does not belong to us.}

\item[$\bullet$] \textit{Step 2:} We send an HTTP request to the CDN ingress node IP with the custom domain set in CDN as the Host header. If the response contains the correct webpage, that indicates the CDN is vulnerable to domain borrowing.

\item[$\bullet$] \textit{Step 3:} \lzy{For CDN providers vulnerable to domain borrowing, we send an HTTP request to the ingress node IP with a randomly generated non-CDN-deploy domain as the Host header.} We extract the unique HTTP headers and HTTP body from its HTTP response as the non-CDN-deployed fingerprints (as shown in Table~\ref{table: non-CDN-deployed fingerprints}).
% (e.g., random.non-deployed.com) 

\end{itemize}


\noindent \textbf{Generating HTTP requests and recognizing borrowing domains.}
Firstly, we use the previously collected domains not hosted by CDN as the Host headers to generate HTTP requests. Secondly, we send HTTP requests to the ingress node IPs. However, to not burden the CDN services with the following measuring, we select one ingress node IP from each city as a set representing all ingress node IPs. 
Thirdly, we compare HTTP responses with non-CDN-deployed fingerprints. A mismatch indicates that the domain is borrowing.


\begin{table}[h]
\caption{Non-CDN-deployed fingerprints.}
\footnotesize
\begin{threeparttable}
\begin{tabular}{lcl}
\toprule[1.5pt]
\textbf{CDN}            & \textbf{Code\textsuperscript{2}} & \textbf{Fingerprint\textsuperscript{3}}           \\ 
\midrule
Azion          & 404              & B: Not Found                              \\
Bunny          & 403              & B: Domain suspended or not configured          \\
Cachefly       & 403              & B: Hostname not configured                     \\
CDN77          & N/A              & N/A                                         \\
CDNetworks     & N/A              & N/A                                         \\
CDNsun     & 400              & B: 400 Bad Request                                         \\
ChinaNetCenter & N/A              & N/A                                         \\
CloudFront     & 403              & B: The request could not be satisfied   \\
DogeCloud      & 404              & H: X-Cache-Lookup: Return Directly             \\
EdgeNext       & 403              & B: ERROR: ACCESS DENIED                        \\
Edgio          & 404              & B: 404 - Not Found                             \\
Fastly         & 500              & B: Fastly error: unknown domain           \\
Goooood        & 400              & B: /unkonwdomain404/notfound                   \\
KeyCDN         & 403                 & B: the resource has been denied \\
KuoCai         & 403                 & H: Byte-Error-Code: 0060 \\
Layun          & 200              & B: Error in website request\textsuperscript{4} \\
LightCDN       & 400              & B: 400 Bad Request                             \\
Medianova      & N/A              & N/A                                         \\
Netlify        & 404              & B: Not Found - Request ID                     \\
StackPath      & N/A              & N/A                                            \\
Sudun          & 200              & B: Please use the domain name to access\textsuperscript{4} \\ 
UCloud         & 403              & B: ERROR: ACCESS DENIED                        \\
Udomain        & 503              & B: UDomain CDN | Error 503                     \\
Yundun         & N/A              & N/A                                         \\
\bottomrule[1.5pt]
\end{tabular}
\begin{tablenotes}
\item [1] N/A means that the CDN does not respond to the request.
\item [2] Code means HTTP response status codes.
\item [3] Fingerprint types: B=HTTP Body, H =HTTP Header.
\item [4] In most cases, the returned fingerprits are in English.
\end{tablenotes}
\end{threeparttable} 
\label{table: non-CDN-deployed fingerprints}
\end{table}




\subsection{Domain Takeover Detector}
Figure~\ref{fig: workflow} shows the workflow of Domain Takeover Detector, which can be divided into three steps: (1) We identify vulnerable CDNs and collect HTTP responses of the domain stopped its CDN service as CDN-service-discontinued fingerprints. (2) We use the previously collected domain data to discover domains hosted by vulnerable CDNs. (3) We send HTTP requests to domains hosted by vulnerable CDNs and compare HTTP responses with CDN-service-discontinued fingerprints.

\noindent \textbf{Identifying vulnerable CDNs.}
To identify CDNs vulnerable to domain takeover, we investigated their domain connection and domain verification mechanism. Firstly, we reviewed the documentation provided by CDN providers and searched for tutorial videos on service configurations to understand the officially stated domain verification mechanism. 
\lzy{Secondly, we registered two test accounts\footnote{We registered two test accounts to verify that the CDN vendors did not perform the domain verification mechanism or that they performed the flawed domain verification mechanism. This only confirms DVA vulnerability and does not impact the automation of \toolname.} for each CDN provider to validate the feasibility of domain takeover in practice. Step 1: we use an account (as a victim) to create a CDN service and add DNS records to deploy a domain in CDN. Step 2: we delete the CDN service to make the victim's domain dangling. Step 3: we use another account (as an attacker) to create a CDN service and attempt to take over the victim's dangling domain.}
Previous research~\cite{understand_dns_threat,takeover_xyz,dare_shark} has primarily focused on widely used web-hosting services, but systematic testing of CDN has not been fully conducted. To fill this gap, we systematically explored the practices currently adopted by CDNs and identified 19 vulnerable CDNs. 
\lzy{Additionally, we discovered new vulnerabilities in the domain verification mechanism. Details of exploiting these vulnerabilities for domain takeover are in Section~\ref{subsec: Newfindings}.}
When a CDN service is deactivated, the CDN responds to the client with distinctive HTTP or DNS responses. We collected these responses as CDN-service-discontinued fingerprints to determine service status and detect dangling domains. Throughout the research process, we summarized three types of fingerprints (in Table~\ref{talbe: CDN service discontinuation fingerprints}):

\begin{itemize}

\item[$\bullet$]HTTP response headers. 
These are essential for assessing the status of a domain. CDNs typically use default HTTP error codes, like ``404 Not Found'' to indicate the unavailability of services. To differentiate between service discontinuation and other types of failures, we also extract specialized HTTP headers from each service alongside status codes. 

\item[$\bullet$]HTTP response bodies. 
CDNs often employ default error pages with similar HTML structures or specific notification phrases to indicate service status. We utilize the typical content of these pages as fingerprints, such as the phrase ``Fastly error: unknown domain'' to identify service discontinuation, following methodologies from previous research~\cite{takeover_xyz}.

\item[$\bullet$]DNS responses.
CDNs may deliver customized DNS responses when a domain's service is canceled. For instance, domains might resolve to specific IP addresses, such as 127.0.0.1. In cases where the service is discontinued and caches have expired, assigned sub-domains may return non-existent domain errors (i.e., NXDOMAIN).

\end{itemize}


\noindent \textbf{Discovering domain hosted by vulnerable CDNs and recognizing dangling domains.}
Firstly, to discover domains hosted by vulnerable CDNs, the Domain Takeover Detector analyzes domains' DNS records to verify whether they match the fingerprints of CDN providers previously identified as vulnerable to domain takeover. 
Secondly, the Domain Takeover Detector compares the DNS responses provided by CDN Checker with CDN-service-discontinued fingerprints. If there is no match, the Domain Takeover Detector sends HTTP requests to the domain and compares the HTTP responses with  CDN-service-discontinued fingerprints. Ultimately, domains with matched CDN-service-discontinued fingerprints are considered dangling domains.

\begin{table}[ht]
\caption{CDN-service-discontinued fingerprints.}
\footnotesize
\begin{threeparttable}
\begin{tabular}{lcl}
\toprule[1.5pt]
\textbf{CDN}                     & \textbf{Code\textsuperscript{2}} & \textbf{Fingerprint\textsuperscript{3}} \\
\midrule
Azure        & NA              & D: NXDOMAIN         \\
Bunny         & 403              & B: Domain suspended or not configured       \\
Cachefly       & 404              & B: hostname not configured                   \\
CDNetworks     & NA               & D: NXDOMAIN                                 \\
ChinaNetCenter & NA               & D: NXDOMAIN                                 \\
Cloudflare     & 530                 & \makecell[l]{ B: Cloudflare is currently unable \\to resolve your requested domain}                                            \\
DogeCloud          & 404              & H: X-Cache-Lookup: Return Directly                             \\
EdgeNext       & NA               & only have one A record.                     \\
Edgio        & 404              & H\&B: 404 - Not Found                             \\
Fastly        & 500              & B: Fastly error: unknown domain          \\
G-core         & NA               & D: SERVFAIL                              \\
KuaikuaiCloud         &NA                & D: 127.0.0.1                                \\
KuoCai         & NA               & D: NXDOMAIN                                 \\
Layun          & 200              & B: Error in website request\textsuperscript{4} \\
LightCDN       & NA               & D: NXDOMAIN                                 \\
Netlify        & 404              & B: Not Found - Request ID                   \\
Sudun          & 200              & B: Please use the domain to access\textsuperscript{4} \\ 
UCloud         & NA               & D: NXDOMAIN                                 \\
Yundun         & NA               & D: NXDOMAIN                                 \\
\bottomrule[1.5pt]
\end{tabular}

\begin{tablenotes}
\item [1] N/A means that the CDN does not respond to the request.
\item [2] Code means HTTP response status codes.
\item [3] Fingerprint types: D=DNS Response, B=HTTP Body, H=HTTP Header.
\item [4] In most cases, the returned fingerprints are in English.
\end{tablenotes}
\end{threeparttable} 
\label{talbe: CDN service discontinuation fingerprints}
\end{table}


